A Generalized Algorithm for Multi-Objective Reinforcement Learning and Policy Adaptation

We introduce a new algorithm for multi-objective reinforcement learning (MORL) with linear preferences, with the goal of enabling few-shot adaptation to new tasks. In MORL, the aim is to learn policies over multiple competing objectives whose relative importance (preferences) is unknown to the agent. While this alleviates dependence on scalar reward design, the expected return of a policy can change significantly with varying preferences, making it challenging to learn a single model to produce optimal policies under different preference conditions. We propose a generalized version of the Bellman equation to learn a single parametric representation for optimal policies over the space of all possible preferences. After an initial learning phase, our agent can execute the optimal policy under any given preference, or automatically infer an underlying preference with very few samples. Experiments across four different domains demonstrate the effectiveness of our approach.

==> app-ttest.tex <==
\subsection{Tests of Significance}

Here we performed the unpaired t-test between our envelope model and other three MORL baselines, over 5 independent runs for each algorithm on each domain. The one-sided p-values are shown in Table~\ref{tbl:ttest}. We achieved significance scores of $p<0.05$ vs MOFQI on all domains, $p<0.01$ vs CN+OLS on DST and $p<0.05$ vs Scalarized on FTN, Dialog and SuperMario. % We will add this information to the results table. 

% The following table, corresponding to Table~\ref{tab:overall}, reports {\bf one-sided p-value from unpaired t-test} comparing our envelope algorithm with other three MORL baselines, over 5 independent runs for each algorithm on each domain.
\begin{table}[h]
    \centering
    \vspace{-.2em}
    \caption{One-sided P-value from unpaired t-test for performance comparison among Envelope (ours) and other MORL algorithms.}
    \resizebox{\columnwidth}{!}
    {
        \setlength{\tabcolsep}{1pt}
        \begin{tabular}{ccccccc}
    	\toprule
		\multirow{2}{3em}{Comparison} & \multicolumn{2}{c}{DST} 
		       & \multicolumn{2}{c}{FTN ($d=6$)} 
		       & \multicolumn{1}{c}{Dialog} 
		       & \multicolumn{1}{c}{SuperMario}\\
		\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}
		{} & {\tt CR} (greater) & {\tt AE} (less) & {\tt CR} (greater) & {\tt AE} (less) & {\tt Avg.}{\tt UT} (greater) & {\tt Avg.}{\tt UT} (greater) \\
		\midrule
		Envelope v.s. MOFQI & 0.066
		 & 8.588$\times$10$^{-4}$ & 5.986$\times$10$^{-8}$
		 & 2.054$\times$10$^{-17}$ & 0.004
		 & -
        \\
		Envelope v.s. CN+OLS & 0.015
		 & 3.254$\times$10$^{-7}$ & -
		 & - & 0.207
		 & -
        \\
		Envelope v.s. Scalarized & 0.333
		 & 0.389 & 0.008
		 & 0.005 & 0.044
		 & 0.038
        \\
		\bottomrule
    \end{tabular}
    \vspace{-.5em}
    }
    \label{tbl:ttest}
\end{table}

% We performed the unpaired t-test between our envelope model and the baselines and achieved significance scores of $p<0.05$ vs MOFQI on all domains, $p<0.01$ vs CN+OLS on DST and $p<0.05$ vs Scalarized on FTN, Dialog and SuperMario. We will add this information to the results table. 


==> experiments.tex <==
\section{Experiments}
\label{s:experiments}
% \karthik{do we compare with prior work?}

We first describe two quantitative evaluation metrics we use and then detail our experiments on three different domains. We leave specific model architecture and other implementation details to the supplementary material.
\subsection{Evaluation Metrics}
\label{sec:metrics}
We use two quantitative metrics to evaluate the empirical performance of our algorithms:

\textbf{Coverage Ratio (CR)}
\label{sec:eval-metic:cr}
The first metric is \textit{coverage ratio} (CR), which evaluates the agent's ability to recover optimal solutions in the convex coverage set ($\mathtt{CCS}$). If $\mathcal F \subseteq \mathbb R^{m}$ is the set of solutions found by the agent (via sampled trajectories),
% and $\mathcal F_{Q} \subseteq \mathbb R^{m}$ is the set of agent's guessed solutions (via predictions from Q-network), 
we define $\mathcal F \cap_{\epsilon}\mathtt{CCS}:=\{x\in \mathcal F \mid \exists y \in \mathtt{CCS} \textrm{~s.t.~} \|x-y\|_{1}/\|y\|_1 \leq \epsilon \}$ as the intersection between these sets with a tolerance of $\epsilon$. 
The CR is then defined as:
\begin{equation}
    \mathtt{CR_{F1}}(\mathcal F) = \mathtt{2} \cdot \frac{ \mathtt{precision\cdot recall}}{\mathtt{precision} + \mathtt{recall}},
\end{equation}
where the $\mathtt{precision} = |\mathcal F \cap_{\epsilon} \mathtt{CCS}|/|\mathtt{\mathcal F}|$, indicating the fraction of optimal solutions among the retrieved solutions, and the $\mathtt{recall} = |\mathcal F \cap_{\epsilon}\mathtt{CCS}|/|\mathtt{CCS}|$, indicating the fraction of optimal instances that have been retrieved over the total amount of optimal solutions (see Figure~\ref{fig:eval-metric}(a)).
% The F1 score is their harmonic mean. 
% In our evaluation of all the three synthetic tasks, we set $\epsilon = 0.00$ for $\mathcal F_{\Pi_{\mathcal L}}$ and $\epsilon = 0.20$ for $\mathcal F_{Q}$. 
% Figure \ref{fig:eval-metric} (a.) illustrates an example of the computation of coverage ratio.

\textbf{Adaptation Quality (AQ)}
\karthik{Update to new definition?}
\label{sec:eval-metic:aq}
Our second metric compares the retrieved control frontier with the optimal one, when an agent is provided with a specific preference $\bm\omega$ during the adaptation phase. 
The adaptation quality is defined by
\begin{equation}
    \mathtt{AQ}(\mathcal C) = \frac{1}{1+ \alpha \cdot \mathtt{err}_{\mathcal D_{\omega}}},
\end{equation}
where the $\mathtt{err}_{\mathcal D_{\omega}} = \mathbb E_{\bm \omega \sim \mathcal D_{\omega}} [|\mathcal C(\bm \omega) - \mathcal C_{\textrm{opt}}(\bm \omega)| / \mathcal C_{\textrm{opt}}(\bm \omega)]$ is the expected relative error between optimal control frontier $\mathcal C_{\textrm{opt}}: \Omega \rightarrow \mathbb R$ with $\bm \omega \mapsto \max_{\bm{\hat r}\in \mathtt{CCS}} \bm \omega^{\intercal} \bm{\hat r}$ and the agent's control frontier $\mathcal C_{\pi_{\bm \omega}} = \bm \omega^{\intercal} \bm{\hat r}_{\pi_{\bm \omega}}$ , and $\alpha$ is a scaling coefficient to amplify the discrepancy. 


% The optimal {\em control frontier} of the problem is defined by a function  $\mathcal C_{\textrm{opt}}: \Omega \rightarrow \mathbb R$ with $\bm \omega \mapsto \max_{\bm{\hat r}\in \mathtt{CCS}} \bm \omega^{\intercal} \bm{\hat r}$. Similarly, $\mathcal C_{\pi_{\bm \omega}} = \bm \omega^{\intercal} \bm{\hat r}_{\pi_{\bm \omega}}$ is the control frontier an agent can achieve (via sample trajectories), and $\mathcal C_{Q}$ is the control frontier guessed by an agent (via predictions from Q-network).

%In all experiment domains, we use Gaussian distributions which are restricted to be positive part and $\ell1$-normalized as our $\mathcal D_{\omega}$ and set $\alpha = 10.0$. 
Figure \ref{fig:eval-metric} (b.) shows examples of optimal control frontier, retrieved control frontier, and the control discrepancy.
Overall, CR provides an indication of agent's ability to learn the space of optimal policies in the learning phase, while AQ tests its ability to adapt to new scenarios.

\begin{wrapfigure}{R}{0.5\textwidth}
    \includegraphics[width=0.48\columnwidth]{figure/metric}
%    \vspace{-1.5em}
    \caption{Quantitative evaluation metrics for multi-objective reinforcement learning. (a.) Coverage ratio measures an agent's ability to find all the potential optimal solutions in the convex coverage set of Pareto frontier.  (b.) Adaptation quality measures an agent's ability of policy adaptation to real-time specified preferences.}
%   	\vspace{-1em}
    \label{fig:eval-metric}
\end{wrapfigure}


% \subsection{Domains}
% \label{sec:env}

\subsection{Fruit Tree Navigation (FTN)}
\label{sec:env:ftn}
Our first domain is a synthetic full binary tree of depth $d$ with randomly assigned vectorial reward $\bm r\in \mathbb R^6$ on the leaf nodes (Figure~\ref{fig:ftn-env}). These rewards encode the amounts of six different components of nutrition of the {\em fruits} on the tree: $\{\mathtt{Protein}, \mathtt{Carbs}, \mathtt{Fats}, \mathtt{Vitamins}, \mathtt{Minerals}, \mathtt{Water}\}$. The rewards are generated such that each node lies on the $\mathtt{CCS}$, i.e. for every node, $\exists \bm \omega$ for which it is optimal. The goal of our MORL agent is to find a path from the root to a leaf node that maximizes utility for a given preference, choosing between left or right subtrees at every non-terminal node. Even though the task is synthetic, it allows us to concretely measure performance of our algorithms since we have complete knowledge of the optimal set of policies. 

\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{figure/ftn-env}
%    \vspace{-1.5em}
    \caption{Fruit Tree Navigation (FTN):  An agent travels from the root node to one of the leaf node to pick a fruit according to a post-assigned preference $\bm \omega$ on the components of nutrition, treated as different objectives. The observation of an agent is its current coordinates $(\mathtt{row}, \mathtt{col})$, and its valid actions are moving to the left or the right child node.}
%    \vspace{-1em}
    \label{fig:ftn-env}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figure/syn-vis-small}
%    \vspace{-1.5em}    
    \caption{Comparison of CCS and control frontiers of deep MORL algorithms. The left figure is visualizing the real CCS and retrieved CCS of scalarized and envelope MORL algorithms using t-SNE. The right figure presents the slices of optimal control frontier and the control frontier of scalarized and envelope MORL algorithms along the $\mathtt{Mineral}$-$\mathtt{Waters}$ plane.}
    \label{fig:syn-vis}
\end{figure}

\begin{figure*}[t]
	\centering
	\includegraphics[width=\textwidth]{figure/syn-exp-results}
%	\vspace{-1.5em}
	\caption{Coverage Ratio (CR) and Adaptation Quality (AQ) comparison of the scalarized deep MORL algorithm and the envelope deep MORL algorithm tested on fruit tree navigation tasks of depths $d= 5, 6, 7$. Trained on 5000 episodes.}
%	\karthik{make labels bigger. }
%	\vspace{-1em}
	\label{fig:sample-ft}
\end{figure*}


\paragraph{Sample Efficiency}
\label{sec:syn-exp:sample}
To compare sample efficiency during the learning phase, we train both our scalarized and envelope deep MORL on the FTN task with depth 6 for 5000 episodes. We compute covereage ratio (CR) over 2000 episodes and adaptation quality (AQ) over 5000 episodes. Figure~\ref{fig:sample-ft} (blue and orange curves) shows plots for the metrics computed over a varying number of sampled preferences $N_{\omega}$ (more details can be found in the supplementary material). Each point on the curve is averaged over 5 experiments. We observe that the envelope MORL algorithm consistently has a better CR and AQ scores than the scalarized version, with smaller variances. As $N_{\omega}$ increases, CR and  AQ both increase, which shows better use of historical interactions for both algorithms when $N_{\omega}$ is larger. This reinforces our theoretical analysis that the envelope MORL algorithm has better sample efficiency than the scalarized version.

% We compare the sample efficiency of the scalarized and envelope version deep MORL algorithms in the {\em Fruit Tree Navigation} (FTN) task with the depth of the tree is $d=6$. 
% We trained our algorithms for 5000 episodes and evaluate their coverage ratios (CR) on 2000 episodes with randomly sampled preferences, and their adaptation qualities (AQ) on 5000 episodes. 
% We fix the number of interactions in this environment, and varies the number of sampled preferences $N_{\omega}$ for updating models in both algorithms. We increase $N_{\omega}$ from $1$ to $128$. The implementation detail can be found in Appendix \ref{app:experiments}. 

% Figure \ref{fig:sample-ft} (a) compares their coverage ratios (blue and orange curves). Each point on the curve is an average of 5 experiments. The envelope deep MORL algorithm has better coverage ratio than the scalarized version for all numbers of sampled preferences, and has relatively lower variances.  
% Figures \ref{fig:sample-ft} (b) and (c) compare our algorithms' adaptation quality during prediction and execution. 
% For all numbers of sampled preferences, the envelope deep MORL algorithm has better execution AQ than the scalarized algorithm. 
% %Even though we know there is a better CR of the envelope version, this result indicates the envelope version algorithm has better alignment between preferences and policies. 
% %As $N_{\omega}$ increases, the values of execution AQ and prediction AQ of both algorithms keep increase. 
% As $N_{\omega}$ increases, the CR and the both AQ values increase, which verifies a better use of historical interactions for both algorithm when $N_{\omega}$ is larger. 
% %Notice that even though when $N_{\omega} = 1$ the execution AQ of the scalarized version and the envelope version differ only around $0.05$, when $N_{\omega}$ increase to $4$, the envelope version algorithm better utilizes the sampled preferences to improve the execution AQ to above 0.9. 
% This agrees with our theoretical analysis that our envelope deep MORL algorithm has better sample efficiency than the scalarized version.

\paragraph{Scalability}
\label{sec:syn-exp:sample}
Figure~\ref{fig:sample-ft} also contains curves for two more FTN environments with $d=5$ (with 32 solutions) and $d=7$ (with 128 solutions). We observe that both scalarized and envelope algorithms are close to optimal when $d=5$ but both CR and AQ values are low for $d=7$. However, the envelope version is more stable and outperforms the scalarized MORL algorithm in both cases. As $N_{\omega}$ increases, the scores of both algorithms increase.  These results point to the robustness and scalability of our algorithms.

% The prediction ability will also be improved as $N_{\omega}$ increases, which means our method is robust in the learning phase to the size of CCS.


% We also investigate the effect of the size of the optimality frontier on algorithm performance. Specifically, we train on two more FTN environments with $d=5$ (which has 32 solutions) and $d=7$ (which has 128 solutions). Figure \ref{fig:sample-ft} (a) shows the results of coverage ratio evaluation. Both scalarized and envelope algorithms work well when $d=5$ and the CR F1 scores are very close to 1, but both of them work badly well when $d=7$. 
% The envelope version algorithm is more stable and outperform the scalarized MORL algorithm on both case. Besides, the envelope deep MORL algorithm can predict multi-objective solutions, while the scalarized algorithm cannot. The prediction ability will also be improved as $N_{\omega}$ increases, which means our method is robust in the learning phase to the size of CCS.



% We also investigate how the size of optimality frontiers will affect the performance of our algorithms. We train our deep MORL algorithms on two new FTN environments with $d=5$ (which has 32 solutions) and $d=7$ (which has 128 solutions) respectively. 
% One is smaller than the previous environment, which contains only $32$ optimal solutions, the other is larger than the previous environment, containing $128$ solutions on the CCS. 

% As for the adaptation quality, Figures \ref{fig:sample-ft} (b) and (c) show the envelope deep MORL algorithm in simpler environment can reach above 0.9 execution AQ by sampling few preferences each update. It verifies the better sample efficiency of the envelope version algorithm. In the harder task the envelope version is constantly better than the scalarized version. Moreover, as $N_{\omega}$ increases, the execution AQ and the prediction AQ of both algorithms increase. And the envelope version algorithm gains greater improvements. These results support the robustness and scalability of our algorithms.


\paragraph{Visualizing frontiers}
\label{sec:syn-exp:visulization}
We also provide a visualization of the convex coverage set (CCS) and control frontier for our algorithms in Figure~\ref{fig:syn-vis}. 
% Figure \ref{fig:syn-vis} illustrates the comparison of CCS and control frontier of deep MORL algorithms. Both figure (a.) and (b.) are measured on a fruit tree navigation task with the depth of 6 which contains total 64 solutions in the real CCS.
The left figure shows the real CCS and retrieved CCS of both MORL algorithms using t-SNE \citet{t-SNE}. We observe that the envelope algorithm (green dots) almost completely covers the entire set of optimal solutions in the real CCS whereas the scalarized algorithm (pink dots) does not. 
The right figure presents the slices of optimal control frontier and the control frontier of our algorithms along the $\mathtt{Minerals}$-$\mathtt{Water}$ plane. The envelope version retrieves almost the entire optimal frontier, while the scalarized version algorithm has larger control discrepancies. The small discrepancy between the real control frontier and the one retrieved by envelope version algorithm at the indentation of the frontier indicates an alignment issue between the preferences and optimal policies. 

% However, there is a small discrepancy between the real control frontier and the one retrieved by envelope version algorithm at the indentation of the frontier. This indicates an alignment issue between the preferences and optimal policies. 


% associating with a desired combination of nutrition. The preferred optimal leaf node has the best utility under a certain given preference. Figure \ref{fig:ftn-env} shows an instance of the {\em fruit tree navigation} task when $d=6$.

%, in which every non-leaf node is associated with zero reward and every fruit is a potential optimal solution in the convex cover set of the Pareto frontier. To construct this, we sample $\bm r^{(i)} = (\bm v^{(i)}_{+} + \bm v^{(i)}_{-})/ \|\bm v^{(i)}\|_{2}$, where $\bm v^{(i)}\sim \mathcal N_{6}(\bm 0,\bm I)$, for each fruit $i$ on a leaf node. The optimal multiple-policy model for this tree structured MOMDP should contain all the paths from the root to different desired fruits. In experiments, we also test on $d=5$ and $d=7$ cases.
%
%In such a simple multi-objective environment, an optimal policy can be easily learned if we know the preference function $f_{\bm \omega}(\cdot ) = \langle \bm \omega, \cdot \rangle$ for scalarization. However, here we are interested in evaluating whether a multiple-policy neural network, trained with deep MORL algorithms, can find and maintain all the potential optimal policies (i.e., paths to every leaf node) when the preference function is unknown, and adapt to the optimal policy when a specific preference is given for execution. 







\subsection{Task-Oriented Dialog Policy Learning}
\label{sec:env:dialog}
Our second experiment domain is task-oriented dialog, where the goal is to learn a policy over agent responses  to a human in order to complete a specific task. In the traditional setup for this task, the rewards are scalar, which does not allow for adapting policies to individual user preferences. 
% Finding a good trade-off between multiple potentially competing objectives is usually domain-specific and not straightforward. 
% For example, in the case when the objectives are brevity and success, if the relative importance weight for success is too high, the resulting policy is insensitive to potentially annoying actions such as {\tt repeat()} provided that the dialogue is eventually successful. 
% . In this case the obtained optimal policy cannot fit all users' preference, and sometimes is out of our expectation. 
%For example, different users may have different preferences to the brevity and the success of conversation with dialogue. Some users interact with the task-oriented dialogue system often when they are driving cars. They hope the dialogue system can provide them a concise response in few turns, rather than a long conversation with very precise information.
%Adaptation to user preferences and balancing these objectives is rarely considered. 
%Conversely, if the relative importance weight for success is too small, the learning algorithm may annoy users by offering inappropriate solutions before fully knowing the user’s requirements. 
% Paper \citet{UltesBCMRSWGY17} proposes a structured method, which is equivalent to our scalarized method but without hindsight experience replay, for finding the optimal weights for a multi-objective reward function.
To address this problem, we transform the dialogue learning process into a MORL scenario with vectorized (2-D) rewards:
$
	\bm r_t = \left[\begin{matrix}
        r_t^{\mathtt{turn}} & r_t^{\mathtt{succ}}
    \end{matrix}\right]^{\intercal}
$,
where $r_t^{\mathtt{turn}}$ is a turn penalty for the brevity objective and $r_t^{\mathtt{succ}}$ is a reward provided on successful completion of the task. We train using 3000 dialogues and evaluate on 5,000 dialogues with randomly sampled preferences.
% Typically, $r^{\mathtt{turn}}_t$ is fixed for each turn as a negative constant $R^{\mathtt{turn}}$, while $r^{succ}_t$ equals a positive constant $R^{\mathtt{succ}}$ only when the dialogue terminates and receives a successful user feedback otherwise it equals zero.
%In the learning phase, the linear preference $\bm \omega$ over these two objectives are unknown, while the computational resources are abundant. The task-oriented dialogue system needs to learn all the possible optimal policies with sampled $\bm \omega$'s (achieved by user simulators or collected interactions with real users). While in the execution phase, learning is unaffordable because of the limitation of resources. The task-oriented dialogue system needs to respond the user with a specified user preference. User's utility increase is aligned with the system's utility increase $\bm \omega^{\intercal}\bm r_t$.  
%Comparing with single-objective reinforcement learning methods, where the relative importance weights of the system is always fixed in both learning and execution phases. The system may not learn the optimal responses under certain preferences, or execute following a policy mismatched user's preference therefore the user's utility is low. 
% We apply our two proposed deep MORL algorithms to the dialogue policy learning, and compare to traditional single-objective methods.



\begin{table}[t]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c}
        &Single-(0.5,0.5) & Single-(0.2,0.8) & Single-(0.8,0.2) & Scalarized & Envelope\\
        \hline
    SR & 88.18 $\pm$ 0.90 & 85.30 $\pm$ 0.98 & 87.62 $\pm$ 0.91 & 86.38 $\pm$ 0.95 & {\bf 89.52 $\pm$ 0.85}\\
    \#T & 8.93 $\pm$ 0.13 & 9.40 $\pm$ 0.16 & {\bf 7.42 $\pm$ 0.10} & 8.08 $\pm$ 0.12 & 8.08 $\pm$ 0.12\\
    UT & 2.13 $\pm$ 0.23 & 1.84 $\pm$ 0.23 & 2.53 $\pm$ 0.22 & 2.38 $\pm$ 0.22 & {\bf 2.65 $\pm$ 0.22}\\
    \hline
    AQ  & 0.660 & 0.279 & 0.728 & 0.614 & {\bf 0.814}\\
    \hline
    \end{tabular}
    }
%    \vspace{-0.5em}
    \caption{\small The average success rate (SR), number of turns (\#T), user utility (UT), and adaptation quality (AQ, $\alpha=0.1$) of policies obtained after 3,000 training dialogues.}
%    \vspace{-1.0em}
    \label{tab:dialogue}
\end{table}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\columnwidth]{figure/dialogue-dist-succ2}
%    \vspace{-1.5em}
    \caption{The MORL success-weight curves after 3,000 training dialogues. Each data point is a moving average of closest around 500 dialogues in the interval of around $\pm$ 0.05 weight of success over three trained policies.}
%    \vspace{-1.5em}
    \label{fig:dialogue-dist-succ}
\end{figure}

\paragraph*{Results} 
From Table~\ref{tab:dialogue}, we observe that envelope MORL achieves best success rate (SR) on average, while the single-objective method with equal weight on both dimensions (0.5) achieves competitive performance. However, on metrics of average utility (UT) and adaptation quality (AQ) (with $\alpha=0.1$, envelope MORL is significantly better than the other methods, including scalarized MORL. This again demonstrates that adaptability of envelope MORL to tasks with new preferences.
% The single-objective method with 0.8 success weight has worst performance on success rate eventually. 
% This is might because lack of turn level reward guidance directly optimize for success is very difficult for the single-objective RL learner. 


% is the quantitative evaluation results for different dialogue policy learning methods. 
% We evaluate the average success rate, the average dialogue length, the average user utility, and the adaptation quality (AQ) of policies obtained by single-objective and multi-objective reinforcement learning algorithms after 3,000 training dialogues. 
% The evaluation is performed on 5,000 dialogues with randomly sampled preference. Our results are as follows: 
% First, 
% Second, the single-objective method with 0.2 success weight (emphasizing the brevity more) achieves the shortest dialogue length. 
% While our two deep MORL algorithms perform much better than other two single-objective settings for the average brevity. 
% Third, as for the average user utility, the envelope deep MORL is better than others. 
% The scalarized deep MORL achieves only an average level of the single-objective results. 
% One explanation for this result is that the scalarized deep MORL requires more sessions for training. 
% Appendix \ref{app:experiments} provides more supportive evidence on this statement. 
% Finally, we use the ideal control frontier to compute the adaptation quality (AQ) with $\alpha = 0.1$ for all learned policies, and the envelope version MORL algorithm reaches the highest score. 
% This supports our statement that MORL algorithm can better adapt to different user preferences. Applying MORL algorithm can help us avoid choosing improper relative importance weights for training. 

% \paragraph*{Performance under Different Preferences}
Figure~\ref{fig:dialogue-dist-succ}  shows success rate (SR) curves as we vary the weight of the preference on task completion succes.  The success rates of both MORL algorithms increase as the user's weight on success increases, while the those of the single-objective algorithms do not change. This shows that our MORL methods can adapt gracefully to the user's preference. Furthermore, our envelope deep MORL algorithm outperforms other algorithms whenever success is relatively more important to the user (weight $> 0.5$).

% To demonstrate our algorithm's policy adaptation ability to different user preferences in the execution phase, Figure \ref{fig:dialogue-dist-succ} shows success-weight curves after 3,000 training dialogues. For each curve, each data point is a moving average of closest around 500 dialogues in the interval of around $\pm$ 0.05 weight of success over three trained policies. As shown in this figure, the success rates of the MORL algorithms increase as the user's weight of success increases, while the success rates of the single-objective algorithms do not change. This means that our MORL methods can adapt to the user's preference, while the single-objective methods cannot. Furthermore, our envelope deep MORL algorithm outperforms other algorithms on the success rate when the success objective is relatively more important to the user.


\subsection{Multi-Objective Super Mario Bros}
\label{sec:env:mario}
Our final environment is a version of the popular video game Super Mario Bros. We modify the open-source environment from OpenAI gym~\citet{gym-super-mario-bros} to provide vectorized rewards encoding five different objectives: {\tt x-pos}: value corresponding to the difference in Mario's horizontal position between current and last time point,  {\tt time}: a small negative time penalty, {\tt deaths}: a large negative penalty given each time Mario dies\footnote{Mario has up to three lives in one episode.},  {\tt coin}:  rewards for collecting coins, and {\tt enemy}: rewards for eliminating an enemy. We use an A3C~\citet{MnihBMGLHSK16} variant of our envelope MORL agent (see supplementary material for details). During the learning phase, the agent does not know the underlying preference, and hence learns a multi-objective policy. During the adaptation phase, our agent performs preference elicitation (as described in Section~\ref{s:inference}) to uncover the underlying preference that maximizes utility.

% To further demonstrate preference elicitation in the analysis phase, we train and test our algorithms in the popular video game Super Mario Bros. Our multi-objective reinforcement learning environment of Super Mario game is modified from one open-sourced OpenAI Gym environment \citet{gym-super-mario-bros}. 
% The state is a stack of four continuous frames of game images rendered by the simulator, and there are seven valid actions each step.
%: \{`NOOP',`right',`right+A',`right+B',`right+A+B', `A', `left'\}, where the button `A' is used to jump and the button `B' is used to run.
% In the learning phase, the game will provide vectorized rewards encoding five different objectives: {\tt x-pos}, the horizontal distance of Mario from the original point. {\tt time}, the time penalty, a small negative constant for every four frames. {\tt life}, the death penalty which is given each time the Mario dies. Mario has up to 3 lives in one episode. {\tt coin}, the reward for coin collection. And {\tt enemy}, the reward for enemy elimination. The the preference over these objectives are unknown to the agent during the learning phase. And in the analysis and execution phases, the agent utilizes the learned trade-offs among objectives in the Mario game to perform preference elicitation algorithm to automatically recover the underlying preference and act optimally.


% We investigate the agent's ability of preference elicitation in a series of variants of Super Mario games $\tt g1$ to $\tt g5$, where only  one single objective is supposed to be maximized.
%The agent is supposed to use the algorithm in Section \ref{s:inference} with its learned policies to infer the underly preferences of these game variants over multiple objectives {\tt x-pos}, {\tt time}, {\tt life}, {\tt coin}, and {\tt enemy} as introduced in Section \ref{sec:env:mario}, from some scalar feedback with only few interactions. 
%When the preference is determined, the agent can perform under the inferred preferences in different game variants.
Table~\ref{tab:mario-enve-infer} shows the learned preferences for 5 different tasks ($\tt g1$ to $\tt g5$) with one-hot preferences $[1,0,0,0,0]$ to $[0,0,0,0,1]$, respectively. These were learned in a few-shot adapation setting, using just 100 episodes. We observe that the learned preferences are concentrated on the diagonal, indicating good alignment with the actual underlying preferences. For example, in the game variant $\tt g4$, the envelope MORL agent finds the preference with highest weight ($0.6960$) on the coin objective can best describe the goal of $\tt g4$, which is to collect as many coins as possible. We also tested policy adaptation on the original Mario game using game scores for the scalar rewards. We find that the agent learns preference weights of 0.37 for {\tt x-pos} and 0.23 for {\tt time}, which is consistent with a common strategy that humans employ -- simply move Mario towards the flag as quickly as possible.

% The results do not exactly match the true preferences, which may be for two reasons: the trade-off frontiers and policy-preference alignments learned by the algorithm may not be perfect, and there may be muliple preferences that result in the same policy and utility. 

% We also deploy the trained envelope MoA3C agents in a Mario Game where only game scores are available. After 100 episodes adaptation, the envelope MoA3C agent infers that the underlying preference for the achieving higher score mainly focuses on {\tt x-pos} (0.3725) and {\tt time} (0.2307), which is coincident with the strategy human players commonly use -- to achieve higher score, especially the stage accomplishment bonus, the first priority is to ensure Mario can move forward towards the flag within the time limit.


% This orthogonal design helps us characterize the behaviors of agents and compare their inferred preferences. We allow agents make 100 episodes interactions in each game variance, to determine the preference. Note that only 100 episodes are far from enough for training a single objective reinforcement learning agent, even the model is pre-trained on other tasks. 

% Tables \ref{tab:mario-enve-infer} shows the results envelope multi-objective A3C (MoA3C) algorithm, the results for scalarized version algorithm is in Appendix \ref{app:experiments}. The preferences inferred by the envelope MoA3C agent is concentrate on the diagonal, which is close to the true underlying preferences. 

%However the scalarized version algorithm incorrectly infers the potential underlying preference and thinks coin objective is the least important. 
% Even though the envelope MoA3C agent indeed can infer preference, our experiments show that the inferred preferences are not exactly the true underlying preferences. It is mainly for two reasons: First, the trade-off frontiers and policy-preference alignment learned by the algorithm is not ideal. There might be some discrepancies between the obtained control frontier and the real optimal control frontier just like what Figure \ref{fig:syn-vis} (b) illustrates. Second, even the agent perfectly learned the frontier and the alignment, close preferences may correspond to the policies with same expected returns.

\begin{table}[t]
	\centering
	\resizebox{0.8\columnwidth}{!}{
	\begin{tabular}{c|c|c|c|c|c}
	& {\tt x-pos} & {\tt time} & {\tt life} & {\tt coin} & {\tt enemy} \\ \hline
  {\tt g1}& \cellcolor{yellow!24}\underline{0.2412} &\cellcolor{yellow!19}0.1901 &\cellcolor{yellow!21}0.2188 &\cellcolor{yellow!23}0.2373 &\cellcolor{yellow!11}0.1123\\ \hline
  {\tt g2}&\cellcolor{yellow!19}0.1985&\cellcolor{yellow!22}\underline{0.2237} &\cellcolor{yellow!24}0.2485 &\cellcolor{yellow!14}0.1422 &\cellcolor{yellow!18}0.1868\\ \hline
  {\tt g3}&\cellcolor{yellow!34}0.3499 &\cellcolor{yellow!08}0.0861 &\cellcolor{yellow!29}\underline{0.2950} &\cellcolor{yellow!15}0.1542 &\cellcolor{yellow!11}0.1147\\ \hline
  {\tt g4}&\cellcolor{yellow!02}0.0211 &\cellcolor{yellow!24}0.2404 &\cellcolor{yellow!02}0.0211 &\cellcolor{yellow!69}\underline{0.6960} &\cellcolor{yellow!02}0.0211\\ \hline
  {\tt g5}&\cellcolor{yellow!07}0.0715&\cellcolor{yellow!10}0.1038 &\cellcolor{yellow!20}0.2069 &\cellcolor{yellow!39}0.3922 &\cellcolor{yellow!22}\underline{0.2253}\\ \hline
	\end{tabular}}
%	\vspace{-0.5em}
	\caption{Inferred preferences of the envelope multi-objective A3C algorithm in different Mario Game variants with 100 episodes.}
	\label{tab:mario-enve-infer}
%	\vspace{-5pt}
\end{table}





% \subsection{Implementation Details}

% \karthik{todo}
% \paragraph{Model Details} Besides, our utility-based multi-objective Q-network can be replaced with any model similar to that in single-objective off-policy RL algorithms like DDPG \citet{LillicrapHPHETS15}, NAF \citet{GuLSL16} or SDQN \citet{MetzIJD17}. Actually, in the experiment, we also use other deep reinforcement learning techniques such as double Q-learning \citet{HasseltGS16} with a target network and prioritized experience replay \citet{SchaulQAS15}, which stabilize and speed up our algorithms a lot. We present the skeleton of our scalarized deep MORL as algorithm \ref{algo:scalarized}.

% \paragraph*{Architectures of the Multi-objective Q-Network} We implement the (utility-based) Multi-objective Q-networks (MQNs) by 4 fully connected hidden layers with  $\{16, 32, 64, 32\} \times (\mathtt{dim}(S)+m)$ hidden unites respectively. The multi-objective Q-networks are similar to Deep Q-Networks (DQNs) \citet{MnihKSRVBGRFOPB15}, but differs on inputs. An input of the  multi-objective Q-network is a concatenation of state representation and parameters of a linear preference function. The output layer of the scalarized MORL algorithm is of size $|\mathcal A|$, and that of envelope version is of size $m\times |\mathcal A|$. Here $\mathtt{dim}(\mathcal S)$ is the dimensionality of the state space, $|\mathcal A|$ is the cardinality of the action set, and $m$ is the number of objectives.
% \karthik{talk  about a3c for mario}

% \paragraph*{Training with Prioritized Double Q-Learning} When training the with our MORL algorithm, we employ techniques of {\em prioritized experience reply} \citet{SchaulQAS15} and {\em double Q-learning} \citet{HasseltGS16} to speed up the training process and to yield more accurate value estimates. Double Q-Learning introduces a target network $Q_{\textrm{target}}$ to replace the estimate of $\mathcal T Q(s, a, \bm \omega)$, $y_t(\bm \omega) = \bm\omega^{\intercal} \bm r + \gamma Q_{\textrm{target}}(s',a,\bm \omega)$ with $y_t^{\textrm{double}}(\bm \omega) = \bm\omega^{\intercal} \bm r + \gamma  Q_{\textrm{target}}(s', \argmax_a Q(s',a,\bm \omega), \bm \omega)$ for scalarized version of algorithm, and similarly we replace $y_t(\bm \omega) = \bm\omega^{\intercal} \bm r + \gamma \bm \omega^{\intercal} \bm Q_{\textrm{target}}(s',a,\bm \omega)$ with $y_t^{\textrm{double}}(\bm \omega) = \bm\omega^{\intercal} \bm r + \gamma \bm \omega^{\intercal} \bm Q_{\textrm{target}}(s', \argmax_a \bm \omega^{\intercal} \bm Q(s',a,\bm \omega), \bm \omega)$ for envelope version of MORL algorithm.  We update the target network by coping from Q-network every $100$ steps. 
% The priority of sampling transition $\tau_i=(s,a, \bm r, s')$ is $p_i^{\textrm{scalarized}}=|y^{\textrm{double}}(\bm \omega) - Q(s, a, \bm \omega)|$ for the scalarized version of MORL algorithm, and similarly $p_i^{\textrm{envelope}}=|y^{\textrm{double}}(\bm \omega) - \bm \omega^{\intercal} \bm Q(s, a, \bm \omega)|$ for the envelope version of algorithm, where $\bm \omega$ is sampled from the distribution $\mathcal D_{\omega}$. When updating the network, a trajectory is sampled by $\tau_{i}\sim P(i) = p_i/\sum_{i}p_i$. The replay memory size is 4000 and the batch size is 32. For the deep tree navigation task, we train each model for total 5000 episodes, and update it by Adam optimizer every step after at least a batch experiences are stored in reply buffer, with a learning rate $\mathtt{lr}=0.001$.

% \paragraph*{Multi-Objective Dialogue Policy Learning}

% The multi-objective reinforcement learning algorithm for task-oriented dialogue policy learning is applied to a restaurant lookup hotline to provide information restaurants in Cambridge. There are 3 search constraints, 9 informational items that the user can request, and 110 database entities. The reward $R^{\mathtt{turn}}$ is $-1$ for each turn, and $R^{\mathtt{succ}} = 20$. The maximal length of dialogue is $25$.

% We use the statistical spoken dialogue toolkit PyDial \citet{UltesRSVKCBMWGY17} to generate dialogue simulations, where an agenda-base user simulator \citet{SchatzmannY09} with an error model to simulate the recognition and understanding errors arisen in the real system due to in the speech noise and ambiguity. All the single-objective and multi-objective reinforcement learning are trained for 3,000 sessions with 15\% simulated error rate. We evaluate learned policies on 5,000 sessions with randomly assigned user preferences. The preference distribution $\mathcal D_{\omega}$ is a truncated Gaussian distribution on a 1-simplex. 

% For the single-objective reinforcement learning algorithms, we set three groups of $\bm \omega$ as $\{(0.5, 0.5),$ $(0.2,0.8),$ $ (0.8,0.2)\}$. For the envelope deep MORL algorithms, the homotopy path is a monotonically increasing track where $\lambda$ increases from $0.0$ to $1.0$ exponentially. The number of sampled preferences $N_{\omega}$ is 32 for both scalarized and envelope deep MORL algorithms. The exploration policy used for training these reinforcement learning algorithms is $\epsilon$-greedy, where $\epsilon = 0.5$ initially and then decays to zero linearly during the training process. For all the single-objective and multi-objective algorithms, we employ the same deep Q-network architecture, which comprises 3 fully connected hidden layers with $\{16, 32, 32\} \times (\mathtt{dim}(S)+m)$ hidden units. The minibatch size is 64 for all. An Adam optimizer is used for updating the parameters of all these algorithms, with an initial learning rate $\mathtt{rl} = 0.001$.

% \paragraph*{MoA3C}
% We use the multi-objective A3C (MoA3C) algorithms for Mario experiment. Both critic and actor networks contain three shared convolutional layers for feature extraction from raw images input. The extracted features are then concatenated with preferences, and fed into two-layer fully connected networks for output. For the scalarized version MoA3C, the output of the critic network is just one-dimensional utility prediction, whereas the output of the envelope version critic network is $m$-dimensional returns prediction. Both scalarized and envelope versions have the same actor network architecture to output the probability distribution over the action space. We train them with 16 workers in parallel with different sampled preferences, and it take around 10 hours for the envelope version MoA3C to converge to a good level of performance.


 


==> results.tex <==
\section{Experimental Results}
\label{s:results}

\subsection{Properties of Deep MORL Algorithms}
\label{sec:results:property}

% \begin{figure*}[t]
% 	\centering
% 	\includegraphics[width=\textwidth]{figure/syn-exp-results}
% 	\caption{Coverage Ratio (CR) and Adaptation Quality (AQ) comparison of the naive deep MORL algorithm and the envelope deep MORL algorithm tested on fruit tree navigation tasks of depths $d= 5, 6, 7$. Trained on 5000 episodes.}
% 	\label{fig:sample-ft}
% \end{figure*}

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\textwidth]{figure/syn-vis}    
%     \caption{Comparison of CCS and control frontiers of deep MORL algorithms. Both figure (a.) and (b.) are measured on a fruit tree navigation task with the depth of 6 which contains total 64 solutions in the real CCS. The left figure is visualizing the real CCS and retrieved CCS of naive and envelope MORL algorithms using t-SNE \cite{t-SNE}. The right figure presents the slices of optimal control frontier and the control frontier of naive and envelope MORL algorithms along the $\mathtt{Mineral}$-$\mathtt{Waters}$ plane.}
%     \label{fig:syn-vis}
% \end{figure*}

% \paragraph{Sample Efficiency}
% \label{sec:syn-exp:sample}

% We compare the sample efficiency of the naive and envelope version deep MORL algorithms in the {\em Fruit Tree Navigation} (FTN) task with the depth of the tree is $d=6$. 
% We trained our algorithms for 5000 episodes and evaluate their coverage ratios (CR) on 2000 episodes with randomly sampled preferences, and their adaptation qualities (AQ) on 5000 episodes. 
% We fix the number of interactions in this environment, and varies the number of sampled preferences $N_{\omega}$ for updating models in both algorithms. We increase $N_{\omega}$ from $1$ to $128$. The implementation detail can be found in Appendix \ref{app:experiments}. 

% Figure \ref{fig:sample-ft} (a) compares their coverage ratios (blue and orange curves). Each point on the curve is an average of 5 experiments. The envelope deep MORL algorithm has better coverage ratio than the naive version for all numbers of sampled preferences, and has relatively lower variances.  
% Figures \ref{fig:sample-ft} (b) and (c) compare our algorithms' adaptation quality during prediction and execution. 
% For all numbers of sampled preferences, the envelope deep MORL algorithm has better execution AQ than the naive algorithm. 
% %Even though we know there is a better CR of the envelope version, this result indicates the envelope version algorithm has better alignment between preferences and policies. 
% %As $N_{\omega}$ increases, the values of execution AQ and prediction AQ of both algorithms keep increase. 
% As $N_{\omega}$ increases, the CR and the both AQ values increase, which verifies a better use of historical interactions for both algorithm when $N_{\omega}$ is larger. 
% %Notice that even though when $N_{\omega} = 1$ the execution AQ of the naive version and the envelope version differ only around $0.05$, when $N_{\omega}$ increase to $4$, the envelope version algorithm better utilizes the sampled preferences to improve the execution AQ to above 0.9. 
% This agrees with our theoretical analysis that our envelope deep MORL algorithm has better sample efficiency than the naive version.

% \paragraph{Robustness to Size of the Frontier}
% \label{sec:syn-exp:sample}

% We also investigate how the size of optimality frontiers will affect the performance of our algorithms. We train our deep MORL algorithms on two new FTN environments with $d=5$ (which has 32 solutions) and $d=7$ (which has 128 solutions) respectively. 
% % One is smaller than the previous environment, which contains only $32$ optimal solutions, the other is larger than the previous environment, containing $128$ solutions on the CCS. 
% Figure \ref{fig:sample-ft} (a) shows the results of coverage ratio evaluation. Both naive and envelope algorithms work well when $d=5$ and the CR F1 scores are very close to 1, but both of them work badly well when $d=7$. 
% The envelope version algorithm is more stable and outperform the naive MORL algorithm on both case. Besides, the envelope deep MORL algorithm can predict multi-objective solutions, while the naive algorithm cannot. The prediction ability will also be improved as $N_{\omega}$ increases, which means our method is robust in the learning phase to the size of CCS.

% As for the adaptation quality, Figures \ref{fig:sample-ft} (b) and (c) show the envelope deep MORL algorithm in simpler environment can reach above 0.9 execution AQ by sampling few preferences each update. It verifies the better sample efficiency of the envelope version algorithm. In the harder task the envelope version is constantly better than the naive version. Moreover, as $N_{\omega}$ increases, the execution AQ and the prediction AQ of both algorithms increase. And the envelope version algorithm gains greater improvements. These results support the robustness and scalability of our algorithms.


% \paragraph{Frontiers Visualization}
% \label{sec:syn-exp:visulization}

% Figure \ref{fig:syn-vis} illustrates the comparison of CCS and control frontier of deep MORL algorithms. Both figure (a.) and (b.) are measured on a fruit tree navigation task with the depth of 6 which contains total 64 solutions in the real CCS. The left figure is visualizing the real CCS and retrieved CCS of naive and envelope MORL algorithms using t-SNE \cite{t-SNE}. From this figure we can see that the envelope version algorithm (dots in green) covers almost every optimal solutions in the real CCS than the naive algorithm (dots in pink). The right figure presents the slices of optimal control frontier and the control frontier of naive and envelope MORL algorithms along the $\mathtt{Mineral}$-$\mathtt{Waters}$ plane. The envelope version algorithm retrieves almost the whole real control frontier, while the naive version algorithm has larger control discrepancies. However, there is a small discrepancy between the real control frontier and the one retrieved by envelope version algorithm at the indentation of the frontier. This indicates an alignment issue between the preferences and optimal policies.


\subsection{Applicability in Dialogue Policy Learning}

% \paragraph*{Success and Brevity Performances} 


% \begin{table}[t]
%     \centering
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{c|c|c|c|c|c}
%         &Single-(0.5,0.5) & Single-(0.2,0.8) & Single-(0.8,0.2) & Naive & Envelope\\
%         \hline
%     SR & 88.18 $\pm$ 0.90 & 85.30 $\pm$ 0.98 & 87.62 $\pm$ 0.91 & 86.38 $\pm$ 0.95 & {\bf 89.52 $\pm$ 0.85}\\
%     \#T & 8.93 $\pm$ 0.13 & 9.40 $\pm$ 0.16 & {\bf 7.42 $\pm$ 0.10} & 8.08 $\pm$ 0.12 & 8.08 $\pm$ 0.12\\
%     UT & 2.13 $\pm$ 0.23 & 1.84 $\pm$ 0.23 & 2.53 $\pm$ 0.22 & 2.38 $\pm$ 0.22 & {\bf 2.65 $\pm$ 0.22}\\
%     \hline
%     AQ  & 0.660 & 0.279 & 0.728 & 0.614 & {\bf 0.814}\\
%     \hline
%     \end{tabular}
%     }
%     \caption{\small The average success rate (SR), number of turns (\#T), user utility (UT), and adaptation quality (AQ, $\alpha=0.1$) of policies obtained by single-objective and multi-objective reinforcement learning algorithms after 3,000 training dialogues.}
%     \label{tab:dialogue}
% \end{table}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{figure/dialogue-dist-succ2}
%     \caption{The MORL success-weight curves after 3,000 training dialogues. We evaluate policies on 5,000 dialogues with near-uniformly randomly sampled preference. For each curve, each data point is a moving average of closest around 500 dialogues  in the interval of around $\pm$ 0.05 weight of success over three trained policies.}
%     \label{fig:dialogue-dist-succ}
% \end{figure}

% Table \ref{tab:dialogue} is the quantitative evaluation results for different dialogue policy learning methods. 
% We evaluate the average success rate, the average dialogue length, the average user utility, and the adaptation quality (AQ) of policies obtained by single-objective and multi-objective reinforcement learning algorithms after 3,000 training dialogues. 
% The evaluation is performed on 5,000 dialogues with randomly sampled preference. Our results are as follows: 
% First, the envelope version MORL algorithm achieves best success rate in average, and the single-objective method with 0.5 weight of success achieves a competitive success rate. 
% The single-objective method with 0.8 success weight has worst performance on success rate eventually. 
% This is might because lack of turn level reward guidance directly optimize for success is very difficult for the single-objective RL learner. 
% Second, the single-objective method with 0.2 success weight (emphasizing the brevity more) achieves the shortest dialogue length. 
% While our two deep MORL algorithms perform much better than other two single-objective settings for the average brevity. 
% Third, as for the average user utility, the envelope deep MORL is better than others. 
% The naive deep MORL achieves only an average level of the single-objective results. 
% One explanation for this result is that the naive deep MORL requires more sessions for training. 
% Appendix \ref{app:experiments} provides more supportive evidence on this statement. 
% Finally, we use the ideal control frontier to compute the adaptation quality (AQ) with $\alpha = 0.1$ for all learned policies, and the envelope version MORL algorithm reaches the highest score. 
% This supports our statement that MORL algorithm can better adapt to different user preferences. Applying MORL algorithm can help us avoid choosing improper relative importance weights for training. 

% \paragraph*{Performance under Different Preferences}

% To demonstrate our algorithm's policy adaptation ability to different user preferences in the execution phase, Figure \ref{fig:dialogue-dist-succ} shows success-weight curves after 3,000 training dialogues. For each curve, each data point is a moving average of closest around 500 dialogues in the interval of around $\pm$ 0.05 weight of success over three trained policies. As shown in this figure, the success rates of the MORL algorithms increase as the user's weight of success increases, while the success rates of the single-objective algorithms do not change. This means that our MORL methods can adapt to the user's preference, while the single-objective methods cannot. Furthermore, our envelope deep MORL algorithm outperforms other algorithms on the success rate when the success objective is relatively more important to the user.


\subsection{Preference Elicitation in Super Mario Game}

% We investigate the agent's ability of preference elicitation in a series of variants of Super Mario games $\tt g1$ to $\tt g5$, where only  one single objective is supposed to be maximized.
% %The agent is supposed to use the algorithm in Section \ref{s:inference} with its learned policies to infer the underly preferences of these game variants over multiple objectives {\tt x-pos}, {\tt time}, {\tt life}, {\tt coin}, and {\tt enemy} as introduced in Section \ref{sec:env:mario}, from some scalar feedback with only few interactions. 
% %When the preference is determined, the agent can perform under the inferred preferences in different game variants.
% This orthogonal design helps us characterize the behaviors of agents and compare their inferred preferences. We allow agents make 100 episodes interactions in each game variance, to determine the preference. Note that only 100 episodes are far from enough for training a single objective reinforcement learning agent, even the model is pre-trained on other tasks. 

% Tables \ref{tab:mario-enve-infer} shows the results envelope multi-objective A3C (MoA3C) algorithm, the results for naive version algorithm is in Appendix \ref{app:experiments}. The preferences inferred by the envelope MoA3C agent is concentrate on the diagonal, which is close to the true underlying preferences. 
% For example, in the game variant $\tt g4$, the envelope MoA3C agent finds the preference with highest weight ($0.6960$) on the coin objective can best describe the goal of $\tt g4$, which is to collect as many coins as possible. 
% %However the naive version algorithm incorrectly infers the potential underlying preference and thinks coin objective is the least important. 
% Even though the envelope MoA3C agent indeed can infer preference, our experiments show that the inferred preferences are not exactly the true underlying preferences. It is mainly for two reasons: First, the trade-off frontiers and policy-preference alignment learned by the algorithm is not ideal. There might be some discrepancies between the obtained control frontier and the real optimal control frontier just like what Figure \ref{fig:syn-vis} (b) illustrates. Second, even the agent perfectly learned the frontier and the alignment, close preferences may correspond to the policies with same expected returns.

% \begin{table}[t]
% 	\centering
% 	\begin{tabular}{c|c|c|c|c|c}
% 	& {\tt x-pos} & {\tt time} & {\tt life} & {\tt coin} & {\tt enemy} \\ \hline
%   {\tt g1}& \cellcolor{yellow!24}\underline{0.2412} &\cellcolor{yellow!19}0.1901 &\cellcolor{yellow!21}0.2188 &\cellcolor{yellow!23}0.2373 &\cellcolor{yellow!11}0.1123\\ \hline
%   {\tt g2}&\cellcolor{yellow!19}0.1985&\cellcolor{yellow!22}\underline{0.2237} &\cellcolor{yellow!24}0.2485 &\cellcolor{yellow!14}0.1422 &\cellcolor{yellow!18}0.1868\\ \hline
%   {\tt g3}&\cellcolor{yellow!34}0.3499 &\cellcolor{yellow!08}0.0861 &\cellcolor{yellow!29}\underline{0.2950} &\cellcolor{yellow!15}0.1542 &\cellcolor{yellow!11}0.1147\\ \hline
%   {\tt g4}&\cellcolor{yellow!02}0.0211 &\cellcolor{yellow!24}0.2404 &\cellcolor{yellow!02}0.0211 &\cellcolor{yellow!69}\underline{0.6960} &\cellcolor{yellow!02}0.0211\\ \hline
%   {\tt g5}&\cellcolor{yellow!07}0.0715&\cellcolor{yellow!10}0.1038 &\cellcolor{yellow!20}0.2069 &\cellcolor{yellow!39}0.3922 &\cellcolor{yellow!22}\underline{0.2253}\\ \hline
% 	\end{tabular}
% 	\caption{Inferred preferences of the envelope multi-objective A3C algorithm in different Mario Game variants with 100 episodes.}
% 	\label{tab:mario-enve-infer}
% \end{table}

% We also deploy the trained envelope MoA3C agents in a Mario Game where only game scores are available. After 100 episodes adaptation, the envelope MoA3C agent infers that the underlying preference for the achieving higher score mainly focuses on {\tt x-pos} (0.3725) and {\tt time} (0.2307), which is coincident with the strategy human players commonly use -- to achieve higher score, especially the stage accomplishment bonus, the first priority is to ensure Mario can move forward towards the flag within the time limit.



